DeepFense: Online Accelerated Defense Against Adversarial Deep Learning

Recent advances in adversarial Deep Learning (DL) have opened up a largely unexplored surface for malicious attacks jeopardizing the integrity of autonomous DL systems. With the wide-spread usage of DL in critical and time-sensitive applications, including unmanned vehicles, drones, and video surveillance systems, online detection of malicious inputs is of utmost importance. We propose DeepFense, the first end-to-end automated framework that simultaneously enables efficient and safe execution of DL models. DeepFense formalizes the goal of thwarting adversarial attacks as an optimization problem that minimizes the rarely observed regions in the latent feature space spanned by a DL network. To solve the aforementioned minimization problem, a set of complementary but disjoint modular redundancies are trained to validate the legitimacy of the input samples in parallel with the victim DL model. DeepFense leverages hardware/software/algorithm co-design and customized acceleration to achieve just-in-time performance in resource-constrained settings. The proposed countermeasure is unsupervised, meaning that no adversarial sample is leveraged to train modular redundancies. We further provide an accompanying API to reduce the non-recurring engineering cost and ensure automated adaptation to various platforms. Extensive evaluations on FPGAs and GPUs demonstrate up to two orders of magnitude performance improvement while enabling online adversarial sample detection.

==> 2_previous.tex <==
%\section{Related Work}
\subsection{Related Work: Adversarial DL}
% Adversarial samples are created from benign samples by adding distortions exploiting the imperfect generalization learned by DNNs from finite training sets. 
Machine learning algorithms are built upon the hypothesis that both the training and test data are collected from the same unknown distributions. Adversarial samples target the imperfect generalization learned by DNNs and thus, violate the aforementioned assumption. Several recent works have focused on devising new attack methodologies with limited attention to possible countermeasures~\cite{szegedy2013intriguing, huang2011adversarial}. The state-of-the-art attacks explore DNN properties that could be used to craft adversarial samples, e.g.,~\cite{goodfellow2014explaining}, ~\cite{nguyen2015deep}. 
%Section XXX provides more details about the mechanisms for crafting malicious inputs. 

To improve the robustness of the DL networks, denoising autoencoders \cite{gu2014towards} were suggested which work by projecting the adversarial samples into the legitimate input space. However, subsequent research has shown that this methodology will not increase the immunity of the victim DL model against the adversaries \cite{} XXX. Other defense methods propose training the network using a supervised learning based on labeled data which includes both benign and malicious samples. The drawback of this methodology is that it can only improve the robustness to the particular noise patterns existing in the labeled data. Another work based on distillation \cite{distillation} aims to improve the robustness by transforming the victim model such that it lies in a smoother gradient space. Unfortunately, this defense has also been shown ineffective against newer adaptive attacks~\cite{carlini2017towards}. 
\mojan{check if distillation is supervised or unsupervised}

It is noteworthy to mention that the works outlined thus far either sacrifice the accuracy of the main DL model or specifically depend on modifying the current DL topology and/or training process. To the best of our knowledge, no prior work targets addressing resource efficiency or online performance of the defense algorithm.

\subsection{Related Work: FPGA Acceleration}
The computation and storage complexity of Deep Neural Network (DNN) models is very high. To improve the accuracy of DNNs, the contemporary literature focus on increasing the model depth, 
which results in a higher number of parameters per network. FPGAs have recently gained significant attention as platform candidates to achieve energy efficient neural network computation alongside CPUs and GPUs~\cite{zhang2015optimizing, sharma2016dnnweaver}. Equipped with DNN-oriented hardware design, FPGAs are able to achieve high parallelism and utilize the properties of neural network (NN) computation to remove unnecessary logic. Algorithmic explorations have shown that neural networks can be simplified to become more hardware friendly without sacrificing the model accuracy~\cite{sze2017efficient}. Therefore, it is possible to achieve a higher energy efficiency on FPGAs compared to CPU and GPU platforms \cite{surveyoffpga} while maintaining the same accuracy. Given a certain FPGA model, the on-chip resource (LUTs, DSPs, BRAMs) are limited. Increasing the peak performance is equivalent to maintaining a high utilization ratio. This can be achieved by implementation of appropriate data parallelism techniques and a suitable memory system \cite{wei2017automated}. Recent research on high-performance NN accelerators has proposed to either reduce the number of weights \cite{zhang2015efficient} or the bit-width used for weight representation \cite{qiu2016going}, which could also help reduce the computation and storage complexity. But these methods can also lead to drops in the model accuracy.
\mojan{make this more compact, mention how what we are doing is fundamentally different from existing work, mention what the challenges are that have not been addressed -> dictionary learning and ..., fine-grained parallelism in the data which we explore by dictionary learning}\\
\mojan{change position od related work to after preliminaries or the end of the paper}
